Multi-view Story Characterization from Movie Plot Synopses and Reviews

This paper considers the problem of characterizing stories by inferring properties such as theme and style using written synopses and reviews of movies. We experiment with a multi-label dataset of movie synopses and a tagset representing various attributes of stories (e.g., genre, type of events). Our proposed multi-view model encodes the synopses and reviews using hierarchical attention and shows improvement over methods that only use synopses. Finally, we demonstrate how can we take advantage of such a model to extract a complementary set of story-attributes from reviews without direct supervision. We have made our dataset and source code publicly available at https://ritual.uh.edu/ multiview-tag-2020.

==> sections/multilabel_evaluation.tex <==
% We evaluate three aspects of the models: a) performance in ranking most relevant tags at the top, b) F1 measure at top $N$ tags, and c) Number of distinct tags predicted in top $N$ tags.
% Previous systems trained on the MPST corpus were evaluated by three metrics: micro-F1, tag recall (TR), and number of distinct tags learned (TL) for the test set.
% Here, micro-F1 gives a sense of the quality of the predictions, TR measures the average recall for each of the tags in the dataset, and TL helps to understand the systems' ability to infer diverse attributes of movies regardless of the imbalance in the dataset.
% Considering the fact that all the target tags have similar weights, measuring the prediction quality with micro-F1 is constrained by the following limitations:
% \begin{itemize}
%     \item Considering the top N tags as predicted tagset, micro-F1 automatically penalizes the samples with target tagset size $\neq$  N.
%     For example, if $N=5$ and a movie has seven target tags, our system will be penalized even if all 5 tags predicted are in the target tags. %despite of having five of them in the top 5 setting, will penalize the system.
%     % Despite the fact that the average target tags per movie is three, having the top 3 tags in the target set penalizes the movies having more than 
%     \item Micro-F1 does not consider the position of predicted tags into consideration. But we argue that a metric that can reward a system for having target tags near the top of the list is more appropriate for this task.  %Having relevant tags appearing near the top of the list is pre
%     %It is necessary to assess the prediction quality %as having a relevant tag at the $N+1st$ position is better than having it for example at the $N+10th$ position.
%     %This issue makes a significant impact in the evaluation due to the incomplete nature of the dataset.
%     %A system that might have ranked more relevant tags than the target tags in the top N prediction, would be penalized.
% \end{itemize}

% Hence, we propose a new metric called \textit{Multi-label Rank (MLR)} that evaluates the prediction quality by considering the ranking of the target tags in models' predictions.
% Multi-label rank of $D$ data samples is defined by
% \begin{equation}
%     mlr = \frac{\sum_{i=1}^{D} (1- \delta_{i})}{D}
% \end{equation}
% %
% Here, $\delta_i$ is the mean \textit{Rank Distance} for an instance $X_i$.
% \textit{Rank Distance} $\delta_{ij}$ for a target tag $t_{ij}\in t_i $ is defined by:
% \begin{equation}
%     \delta_{ij} = \frac{max(0, rank(t_{ij}) - |t_i| + 1)}{|T| - |t_i|}
%     \label{eq:rank_distance}
% \end{equation}
% where, $rank(t_{ij})$ is the ranking position of tag $t_{ij}$ in the predicted ranking of the label set and $|T|$ is the size of label set in the dataset.

% This metric is helpful as it considers all the target tags as equally weighted and results in rank score of $100$ if all of the $K$ target tags are located at the top $K$ positions in the predicted ranking regardless the order of them.
% So the objective for a model becomes to have all the target tags at the top of the predicted ranking in any order to achieve a rank score of $100$.

% % There could be several scenarios where practiced evaluation metrics suffer to assess the classification quality.

% % In this section, we propose a new evaluation metric called \textit{Multi-label rank} for the following multi-label classification scenarios.
% % %
% % \begin{itemize}[leftmargin=0.4cm,labelindent=0cm,noitemsep]
% %     \item Number of labels per sample varies.
% %     \item All the labels for a particular sample are weighted equally.
% %     \item Label density is very low.
% %     \item Objective is to maximize the likelihood of the relevant tags during inference.
% % \end{itemize}
% %


==> tables/gate_activation_percentage.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lcc}
        \toprule
         \textbf{Tag}& \textbf{Narrative} & \textbf{Review}  \\ \midrule
         \texttt{action} & 59.57 & 40.43\\
         \texttt{sadist} & 46.16  &  53.84\\
         \texttt{fantasy} & 62.02  &  37.98\\
         \texttt{cute} & 59.73  &  40.27\\
         \texttt{sentimental} & 59.09  &  40.91 \\
         \texttt{pornographic} & 39.21  &  60.79\\
         \texttt{christian film} & 47.66  &  52.34\\
         \texttt{inspiring} & 53.31  &  46.69\\         
         \bottomrule
    \end{tabular}
    \caption{\small Percentage of gates activated (z $>$ 0.5: narrative; z $<=$ 0.5: review)  movies having specific tags.}
    \label{tab:gate_activation}
\end{table}

==> tables/mlr_progress.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{|c|c|c|}
    \hline
    
    
        \includegraphics[width=0.15\textwidth]{images/epoch_1} &
        % \includegraphics[width=0.15\textwidth]{images/epoch_5} &
        \includegraphics[width=0.15\textwidth]{images/epoch_10} &
        % \includegraphics[width=0.15\textwidth]{images/epoch_15} &
        \includegraphics[width=0.15\textwidth]{images/epoch_20} \\
        % \includegraphics[width=0.15\textwidth]{images/epoch_25} \\ \hline
        % Epoch 1 & Epoch 5 & Epoch 10 & Epoch 15 & Epoch 20 & Epoch 25\\
        \small Epoch 1 & \small Epoch 10 & \small Epoch 20\\
    % MLR: 53.82 & MLR: 86.72 & MLR: 91.42 & MLR: 94.19 & MLR: 96.10 & MLR: 96.42\\
    \small MLR: 53.82, F1: 15.81 & \small MLR: 91.42, F1: 28.18 & \small MLR: 96.10, F1: 46.05\\
        \hline \hline
        
        
        \includegraphics[width=0.15\textwidth]{images/epoch_30} &
        % \includegraphics[width=0.15\textwidth]{images/epoch_35} &
        \includegraphics[width=0.15\textwidth]{images/epoch_40} &
        % \includegraphics[width=0.15\textwidth]{images/epoch_45} &
        \includegraphics[width=0.15\textwidth]{images/epoch_50} \\
        % \includegraphics[width=0.15\textwidth]{images/epoch_60} \\ \hline
    %     Epoch 30 & Epoch 35 & Epoch 40 & Epoch 45 & Epoch 50 & Epoch 60\\ 
    % MLR: 95.30 & MLR: 98.83 & MLR: 98.55 & MLR: 97.36 & MLR: 99.03 & MLR: 99.38\\
    \small Epoch 30 & \small Epoch 40 & \small Epoch 50 \\ 
    \small MLR: 95.30, F1: 55.67 & \small MLR: 98.55, F1: 62.54 &  \small MLR: 99.03, F1: 61.17 \\
    
    \hline
    \end{tabular}}
    \caption{\small Visualization of the Multi-label Rank metric. 
    Each cell presents a plot of the predictions after a particular epoch.
    In each plot, each column represents one data instance and each row represents the rank.
    There are $|Y|$ rows in total.
    The topmost cell in each column represents the class label having the highest probability score predicted by the model that makes it the top ranked class.
    Similarly the bottom-most cell is the lowest ranked class.
    If a cell represents a target class, the cell is colored as \textcolor{blue}{Blue}.
    }
    % \vspace{-1.5em}
    \label{tab:mlr_progress_fig}
\end{table}

==> tables/pretrained_lm_detail_results_val.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{>{\collectcell\mymathrm}l<{\endcollectcell}
>{\collectcell\mymathrm}c<{\endcollectcell}
>{\collectcell\mymathrm}c<{\endcollectcell} >{\collectcell\mymathrm}c<{\endcollectcell}
>{\collectcell\mymathrm}c<{\endcollectcell} >{\collectcell\mymathrm}c<{\endcollectcell}}
\toprule

& & \multicolumn{2}{c}{{$\mathrm{\mathbf{Top 3}}$}} & \multicolumn{2}{c}{\textbf{$\mathrm{\mathbf{Top 5}}$}}\\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}

\multicolumn{1}{c}{} & \multicolumn{1}{c}{$\mathrm{\mathbf{MLR}}$} & \multicolumn{1}{c}{$\mathrm{\mathbf{F1}}$} & \multicolumn{1}{c}{$\mathrm{\mathbf{TL}}$} & \multicolumn{1}{c}{$\mathrm{\mathbf{F1}}$} & \multicolumn{1}{c}{$\mathrm{\mathbf{TL}}$}\\ \midrule

% DistilBERT^H      & 85.98 & 32.24 & 8 & 32.67 & 9\\
% DistilBERT^T      & 85.97 & 32.11 & 8 & 33.00 & 9\\ 
% DistilBERT^{H+T}  & 86.05 & 32.10 & 8 & 33.10 & 11\\
DistilBERT^{S}   & 86.00 & 32.38 & 10 & 32.65 & 10\\
DistilBERT^{O}    & 86.00 & 32.30 & 10 & 32.73 & 10\\
\midrule
% RoBERTa^H      & 88.13 & 34.80 & 20 & 34.95 & 24\\
% RoBERTa^T      & 88.48 & 35.07 & 20 & 35.60 & 27\\
% RoBERTa^{H+T}  & 88.43 & 35.39 & 18 & 35.61 & 26\\
RoBERTa^{S}   & 86.59 & 34.09 & 26 & 34.54 & 29\\
RoBERTa^{O}    & 86.63 & 33.77 & 23 & 34.19 & 28\\
\midrule
% BERT^H      & 88.85 & 35.36 & 24 & 35.92 & 29\\
% BERT^T      & 89.37 & 36.22 & 26 & 36.60 & 30\\ 
% BERT^{H+T}  & 89.28 & 35.95 & 27 & 36.14 & 39\\
BERT^{S}   & \mathbf{88.65} & 35.84 & \mathbf{28} & \mathbf{36.33} & \mathbf{31}\\
BERT^{O}    & 88.29 & \mathbf{36.02} & 23 & 36.25 & 25\\
% BERT^{H+T\dagger}  & 91.78 & 39.14 & 49 & 39.60 & 57\\
BERT^{S\dagger}   & 88.38 & 35.40 & 25 & 35.76 & 29\\
BERT^{O\dagger}    & 88.43 & 35.28 & 22 & 35.99 & 28\\

\bottomrule
\end{tabular}
}
\caption{\small Validation set results using pre-trained language models to extract features from the plot synopses and use that to predict tags. $^S$ denotes sliding window approach without any context and $^O$ denotes overlapping window approach with a context length of 20 tokens. $^\dagger$ denotes fine tuning only the last layer.}
% \vspace{-1.5em}
\label{tab:pretrained_lm_val}
\end{table}







==> tables/results_lm.tex <==
\begin{table*}[!hbtp]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule

& \multicolumn{5}{c}{\textbf{Validation}} & & \multicolumn{5}{c}{\textbf{Test}}\\
% \midrule
\cmidrule(lr){2-6}
\cmidrule(lr){8-12}

& & \multicolumn{2}{c}{{\textbf{Top 3}}} & \multicolumn{2}{c}{\textbf{Top 5}} &  & &\multicolumn{2}{c}{{\textbf{Top 3}}} & \multicolumn{2}{c}{\textbf{Top 5}}
\\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}

\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{MLR}} & \multicolumn{1}{c}{\textbf{Micro F1}} & \multicolumn{1}{c}{\textbf{TL}} & \multicolumn{1}{c}{\textbf{Micro F1}} & \multicolumn{1}{c}{\textbf{TL}}
& & \multicolumn{1}{c}{\textbf{MLR}} & \multicolumn{1}{c}{\textbf{Micro F1}} & \multicolumn{1}{c}{\textbf{TL}} & \multicolumn{1}{c}{\textbf{Micro F1}} & \multicolumn{1}{c}{\textbf{TL}}\\ \midrule
\multicolumn{2}{l}{\textbf{Only Narrative}}& & & &\\ %\hline
Top N$^b$  & 85.23 & 29.70 & 3 & 31.50 & 5 & &
85.66 & 29.70 & 3 & 28.40 & 5 \\

Random N$^b$ & 51.49 & 4.20 & \textit{71} & 5.40 & \textit{71} & &
52.12  & 4.20 & \textit{71} & 6.36 & \textit{71}  \\ %\cline{2-16}

Features$^b$ & 85.23 & 36.90 & 40 & 36.80 & 48 & &
85.66 & 37.30 & 47 & 37.30 &  52  \\ %\cline{2-16}

% #0.377		37		0.376		46
CNN-FE $^b$  & 86.10 & 37.70 &37 & 37.60 & 46 & &
86.51 & 36.90 & 58 & 36.70 & 65\\ 

HAN &  90.94 & 38.89 & 38 & 38.79 & 51 & &
90.85 & 38.25 & 41 & 38.29 & 49   \\

HAN$^\dagger$ &  91.32 & 38.88 & 54 & 39.04 & 61 & &
91.09 & 38.43 & 57  & 38.74 & 64 \\

\multicolumn{2}{l}{\textbf{BERT}} & & & & &\\ %\hline
Head &  88.85 & 35.36 & 24 & 35.92 & 29 & - &- & - & -  & - & - \\
Tail &  89.37 & - & - & - & - & - &- & - & -  & - & - \\
Head+Tail &  89.28 & 35.95 & 27 & 36.14 & 32 & - &- & - & -  & - & - \\
Divide (MP) &  - & - & - & - & - & - &- & - & -  & - & - \\
Slide (MP) &  88.30 & - & - & - & - & - &- & - & -  & - & - \\
\multicolumn{2}{l}{\textbf{RoBERTa}} & & & & &\\ %\hline
Head &  88.13 & - & - & - & - & - &- & - & -  & - & - \\
Tail &  88.48 & - & - & - & - & - &- & - & -  & - & - \\
Head+Tail &  88.43 & - & - & - & - & - &- & - & -  & - & - \\
Divide (MP) &  86.59 & - & - & - & - & - &- & - & -  & - & - \\
Slide (MP) &  86.63 & - & - & - & - & - &- & - & -  & - & - \\


\midrule 
\multicolumn{2}{l}{\textbf{Narrative + Review }} & & & & &\\ %\hline

Concat &  93.36 & 42.46 & 60 & 42.30 & 67 & &
93.19 & 41.96 & 57 & 41.74 & 65 \\ 

Concat$^\dagger$ &  93.31 & 42.78 &60 & 42.80 & 67 & &
93.31 & 41.84 & 60  & 41.79 & 65\\ 

Gate &  93.39 & \textbf{43.60} & 53 & 42.89 & 62  & &
93.23 & 42.28 & 53 & 42.04 & 59\\ 

Gate$^\dagger$  &  93.32 & 42.74 & 60 & 42.29 & 66 & &
93.10 & 41.81 & 59 & 41.67 & 66\\

Gate$^\ddagger$ &  93.50 & 43.36 & 61 & \textbf{43.06} & \textbf{68} & &
\textbf{93.42} & \textbf{42.92} & 60 & \textbf{42.34} & 66\\ 

Gate$^{\dagger\ddagger}$ & \textbf{93.56} & 42.74 & \textbf{63} & 42.52 & \textbf{68} & &
93.38 & 41.90 & \textbf{61} & 41.97 & \textbf{68}\\ 
\midrule
\multicolumn{2}{l}{\textbf{Narrative (LM) }} & & & & &\\ %\hline



\bottomrule
\end{tabular}
}
\caption{\small Results obtained on the validation and test set using different methodologies on the narratives and after adding reviews with the narratives. MLR and TL stand for \textit{multi-label rank} and \textit{tags learned} respectively. $b:$ baseline, $\dagger:$  sentence level prediction enabled,  $\ddagger:$ skip connection enabled.}
\vspace{-1.5em}
\label{tab:resultslm}
\end{table*}

==> tables/summary_human_eval.tex <==
\begin{table}[!]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        
        Baseline & Our System & Tie & Total \\ \hline
        5 & 12 & 4 & 21 \\ \hline
        
        % \multicolumn{4}{|l|}{Helpfulness of closed set tags}\\ \hline
        % Very & Moderate & Not & Total\\ \hline
        % 30 & 29 & 4 & 63 \\ \hline
        
        % \multicolumn{4}{|l|}{Helpfulness of complementary tags}\\ \hline
        % % Extracted tags 141\\
        % 3/3 & 2/3 & 1/3 & 0/3\\ \hline
        % 24\% & 18\% & 32\% & 26\% \\ \hline
        % 3 annotators agreed on 24\%\\
        % 2 annotators agreed on 18\%\\
        % 1 annotators agreed on 32\%
        % Relevant tags 74\%
        
         
    \end{tabular}
    \caption{Summary of the results of the human evaluation.}
    \label{tab:human_eval_summary}
\end{table}{}
